Data augmentation for models based on rejection sampling

We present a data augmentation scheme to perform Markov chain Monte Carlo inference for models where data generation involves a rejection sampling algorithm. Our idea, which seems to be missing in the literature, is a simple scheme to instantiate the rejected proposals preceding each data point. The resulting joint probability over observed and rejected variables can be much simpler than the marginal distribution over the observed variables, which often involves intractable integrals. We consider three problems, the first being the modeling of flow-cytometry measurements subject to truncation. The second is a Bayesian analysis of the matrix Langevin distribution on the Stiefel manifold, and the third, Bayesian inference for a nonparametric Gaussian process density model. The latter two are instances of problems where Markov chain Monte Carlo inference is doubly-intractable. Our experiments demonstrate superior performance over state-of-the-art sampling algorithms for such problems.

==> hoff.tex <==

\subsection{A rejection  sampling algorithm} \label{sec:prior_sim}

We first describe a rejection sampling algorithm from \cite{hoff2009} to draw a sample from the matrix Langevin distribution.
%For parameterizations other than the uniform distribution (i.e.\ for $\bkappa > 0$), even this is non-trivial.
For simplicity, we assume $F$ is orthonormal (i.e.\ that $H$ equals the identity matrix, $I_p$); in the general case, we simply rotate  the resulting draw 
by $H$ (since if $X \sim \ml(\cdot|F)$, then $XH \sim \ml(\cdot|FH^T)$).
%%Consider the matrix Langevin prior on the Stiefel manifold $V_{p,d}$ with parameters $H$ and $\bkappa$.
%%Recall that the matrix Langevin has density given by:
%%\begin{align}
%%  P(X|G, H, \bkappa) &= \etr(H \bkappa G^T X)/Z(\bkappa)
%%\end{align}
%Let $F = G \bkappa H$ be the singular value decomposition of $F$, with the elements of $\bkappa \ge 0$. For simplicity (and as in Section \ref{sec:Bays_inf}), we
%restrict ourselves to
%the case $F = \bkappa H$.
%Recall that we restrict $H^TH = I_p$, additionally, the normalization constant $Z(\bkappa)$ depends only on $\bkappa$.
%We rewrite the prior as
%\begin{align}
%  P(X|H, \bkappa) &= \etr(H^T \bkappa X)/Z(\bkappa)
%We saw in section \ref{sec:param} that
\cite{chikusebook} suggested a simple rejection sampling scheme
based on the envelope:
\begin{align}
  \etr(\bkappa G^T X) & \le \prod_{i=1}^p \exp(\bkappa_i).  \label{eq:chik_bound}
\end{align}
The right-hand side is the mode of $\ml(X|G, \bkappa)$ at $X=G$.
In this scheme, one proposes values uniformly on $V_{p,d}$, accepting a draw $X$ with probability
$\exp(\bkappa G^T X)/\left(\prod_{i=1}^d \exp(\bkappa_i) \right)$.
%Each accepted point is then a sample from the Matrix Langevin distribution.
However, this bound is very loose, making this very inefficient. A rejection sampling algorithm with a significantly
higher acceptance rate was provided in \cite{hoff2009}. Rather than drawing proposals uniformly on $V_{p,d}$, this used the parameters $G$ and
$\bkappa$ to construct a better proposal distribution that we outline in Algorithm \ref{alg:rej_smplr}. At a high level, the algorithm sequentially proposes vectors
from the matrix Langevin on the unit sphere: this is the vector-valued von Mises-Fisher distribution and is straightforward to simulate
\citep{wood1994}.
The mean of the $r${th} vector is $G_{[:r]}$, the $r${th} column of $G$, projected onto $N_r$, the nullspace of the earlier vectors.
Having sampled this $r${th} vector,
it is projected back onto the nullspace $N_r$ and normalized, giving a unit vector orthogonal to the earlier $r-1$ vectors.
This process is repeated $p$ times. Call the resulting
proposal distribution $\seq$; for more details, see \cite{hoff2009}.

{
\vspace{.1in}
\begin{algorithm}[H]
\caption{Proposal distribution $\seq(\cdot|F)$ for matrix Langevin distribution \citep{hoff2009}}\label{alg:rej_smplr}
\begin{tabular}{p{1.4cm}p{12.2cm}}
%\hline
\textbf{Input:}  & The parameters $ F = G\bkappa$ (write $G_{[:i]}$ for column $i$ of $G$) \\
\textbf{Output:} & An output  $X \in V_{p,d}$ (write $X_{[:i]}$ for column $i$ of $X$) \\
\hline
\end{tabular}
\begin{algorithmic}[1]
  \STATE Sample $X_{[:1]} \sim \ml(\cdot|\kappa_i G_{[:1]})$.
  \STATE For $r \in \{2,\cdots p\}$
  \begin{enumerate}[(a)]
    \item Construct $N_r$, an orthogonal basis for the nullspace of $\{X_{[:1]},\cdots X_{[:r-1]} \}$.
    \item Sample $z \sim \ml(\cdot|\kappa_r N^T_r G_{[:r]})$.
    \item Set $X_{[:r]} = z^T N_r/ \|z^T N_r\| $.
  \end{enumerate}
\end{algorithmic}
\end{algorithm}
}

It can be seen that $\seq$ is density on the Stiefel manifold taking the form
\begin{align}
  \seq(X|G, \bkappa) &= \left\{\prod_{r=1}^p \frac{ \|\kappa_r N^T_r G_{[:r]}/2 \|^{(d-r-1)/2 }}{ \Gamma(\frac{d-r+1}{2} ) I_{(d-r-1)/2}(\| \kappa_r N^T_r G_{[:r]} \|)} \right\} \etr(\bkappa G^T X) \label{eq:hoff_seq}\\
               &:= \etr(\bkappa G^T X)/D(X, \bkappa, G) \nonumber
\end{align}
Here, $I_k(\cdot)$ is the modified Bessel function of the first kind. $I_k(x)/x^k$ is an increasing function of $x$,
and  $\|N^T_r G_{[:r]}\| \le \|G_{[:r]}\| = 1$, so that we have the following bound:
\begin{align}
 D(X,\bkappa, G) \le \prod_{r=1}^p  \frac{ \Gamma(\frac{d-r+1}{2} ) I_{(d-r-1)/2}(\| \kappa_r \|)}{ \|\kappa_r/2 \|^{(d-r-1)/2 }} := D(\bkappa) \nonumber
\end{align}
This implies $\etr(\bkappa G^T X) \le D(\bkappa) \seq(X|G,\bkappa) $, which is much tighter than equation \eqref{eq:chik_bound}. %\cite{hoff2009} uses this
We can now construct the following rejection sampler: draw a sample $X$ from $\seq(\cdot)$, and accept it with probability
$D(X, \bkappa, G)/D(\bkappa)$. The set of accepted proposals forms a draw from $\ml(\cdot|G,\bkappa)$, and to obtain samples from $\ml(\cdot|G,\bkappa,H)$,
simply postmultiply these by $H$.

\begin{comment}
While this approach to sampling from the prior is typically adequate, we obtain a different upper envelope to the Matrix Langevin distribution using results
from \citep{Luke1972}.  In that work, two bounds were provided, both ideal for our purposes:
\begin{align}
  \frac{\Gamma(\nu+1)I_{\nu}(x)}{(x/2)^{\nu}} &\le e^x \left( \frac{1}{2\nu + 3} + \frac{2(\nu+1)}{2\nu+3}\left[1 + \frac{2\nu+3)x}{2(\nu+1)}\right]^{-1} \right)\quad x\ge0,\ \nu \ge -1/2,\\
  \frac{\Gamma(\nu+1)I_{\nu}(x)}{(x/2)^{\nu}} &\le \cosh(x) \quad x\ge0,\ \nu \ge -1/2
\end{align}
While, the latter is a bit more convenient, the former is tighter, and we shall use it in the following (referring to it as $b_{\nu}(x)$). For equation \eqref{eq:hoff_seq},
we have the following bound $B(X)$ on $K(X)$:
\begin{align}
 K(X) \le \prod_{r=1}^p  b_{d-r-1}(N^T_r F_{[,r]}) := B(X)
\end{align}
Now, a proposal from $\seq$ is acccepted with probability $K(X)/B(X)$.
By allowing the bound to depend on $X$, we can control the discrepancy between $B(X)$ and $K(X)$ resulting in fewer rejected samples, and greater efficiency.
Note though that our bound $B(X)$ is not uniformly tighter that the bound $B_u$ of \citep{hoff2009}; in particular at the point $X = H$ on the Stiefel manifold,
$B(X) > K(X) = B_u$. On the other hand, our bound has the property that $\inf_{X \in V_{p,d}} K(X)/B(X) > \inf_{X \in V_{p,d}} K(X)/B_u$. This latter property will
be crucial for efficient posterior sampling. Of course, one can always combine the two bounds, defining $\hat{B}(X) = \min (B_u, B(X))$.
%is useful in its own right, providing a more efficient way to sample from the Matrix Langevin. Additionally, our approach will prove crucial for one of our
%algorithms for posterior sampling; with the bound of \cite{hoff2009} being too loose to be practical.
\end{comment}



==> mle.tex <==

We place independent uninformative exponential priors with mean $10$ (and variance $100$) on the scale parameter $\bkappa$, and a uniform prior on the location
parameter $G$. We restrict $H$ to be the identity matrix. Inferences were carried out using the Hamiltonian sampler to produce $10000$ samples, with a
burn-in period of $1000$. For the leapfrog dynamics, we set a step size of $0.3$, with the number of steps equal to $5$.

%The right plot in Figure \ref{fig:vcg_param1} shows the posterior distribution over the first component of $\bkappa$, which is centered around $1.75$
%(the second component is similar).
For comparison, we use the maximum likelihood estimates of the parameters $\bkappa$ and $G$. Obtaining the MLE of
$G$ is straightforward \citep{khatri1977}; %however, the normalization constant $Z(\bkappa)$ makes the MLE of $\bkappa$ harder to estimate.
and for $\bkappa$,
% evaluating the likelihood of the observations is intractable
we follow \cite{khatri1977} and use the approximation of equation \eqref{eq:hgf_asymp} for $Z(\bkappa)$. Performing a grid search over the interval
$0$ to $20$, we obtain ML estimates of % to estimate the components of $\bkappa$.
$11.9$ and $5.9$ for $\kappa_1$ and $\kappa_2$. These are plotted in the right half of Figure \ref{fig:vcg_data} as the red circles, with the blue bars showing the
Bayesian posteriors over these components.
Similarly, the bold straight lines in Figure \ref{fig:vcg_data}(left) show the MLE estimates of the components of $G$, with the small
circles corresponding to $90\%$ Bayesian credible regions
estimated from the MCMC output.
The dashed circles correspond to $90\%$ predictive probability regions for the Bayesian model. To produce these, we generated  $50$ points on $V_{3,2}$ for each MCMC sample,
with parameters specified by that sample. The dashed circles contain $90\%$ of the generated points across all MCMC samples.
%samples for the parameters of
%While MLE of the orientation $G$ agrees with the mode of our Bayesian posterior, we get very large esimates of $\bkappa$ ($11.9$ and $5.9$). These large
%estimates can be attributed to using the asymptotic approximation to the likelihood (as well as the lack of any regularization for the MLE), and results in overconfidence
%in predictions. By contrast, the exact Bayesian approach is robust to these issues.

% \begin{figure}
% \centering
%   \includegraphics[width=.3\textwidth]{figs/plot_vcg_kap1.pdf}
% \centering
%   \includegraphics[width=.3\textwidth]{figs/plot_vcg_kap2.pdf}
%\caption{Posterior distributions over $\kappa_1$, and $\kappa_2$. The red circles are ML estimates.}
% \label{fig:vcg_param1}
% \end{figure}

%MLE:   68.28 + 7.29
%Bayes:  80.01 + 5.26
\begin{table}
\caption{Log predictive-probability of $20$ random held out observations, averaged over $5$ runs.}
\begin{tabular}{|l|l|l|}
\hline
  & MLE & Bayesian inference \\
\hline
Log predictive-probability & $68.78\pm 9.96$ & $78.72 \pm 8.26$ \\
\hline
\end{tabular}
  \label{tbl:cross_val}
\end{table}


% differntiating results in a system of equations that is easy to minimize numerically, and Figure \ref{} show the results.
To quantitatively compare the Bayesian posterior with the ML estimate, we ran a $5$-fold cross-validation,
holding out a random $20$ percent of the observations (call this $X_{test}$), and training the models on the remaining data (call this
$X_{train}$). Table \ref{tbl:cross_val} compares the log probability of the test data under the maximum likelihood estimate, $p(X_{test}|\hat{\bkappa}_{MLE}, \hat{G}_{MLE})$,
with the predictive probability $p(X_{test}|X_{train}) = \int p(X_{test}|\bkappa,G) p(\bkappa,G|X_{train}) \dif \bkappa \dif G$. We approximated
the latter integral by a summation over the MCMC samples, and to evaluate the probabilities $p(X_{test}|\bkappa, G)$ for both methods,
we approximated $Z(\bkappa)$ using equation \eqref{eq:hgf_asymp}.
We see that the log predictive-probability under the Bayesian approach exceeds that of the MLE by about $10$, and demonstrates the importance
of maintaining uncertainty over the matrix Langevin parameters.

%Running our nonparametric analysis on this dataset reveals (as the data suggests) that
%there is no obvious clustering structure, with the data well modelled by a parametric Matrix Langevin distribution. For instance, the
%posterior distribution over the number of clusters is restricted mainly to values less than $2$ (with most probability assigned to $1$).
%In this instance, our nonparametric prior reduces to the simpler parametric distribution. An interesting future direction is to use such ideas to
%build and study nonparametric tests of whether or not the observed data belongs to some parametric family on the Stiefel manifold.

